Understanding Limitation of Two Symmetrized Orders by Worst-case Complexity

Update order is one of the major design choices of block decomposition algorithms. There are at least two classes of deterministic update orders: nonsymmetric (e.g. cyclic order) and symmetric (e.g. Gaussian back substitution or symmetric Gauss-Seidel). Recently, Coordinate Descent (CD) with cyclic order was shown to be $O(n^2)$ times slower than randomized versions in the worst-case. A natural question arises: can the symmetrized orders achieve faster convergence rates than the cyclic order, or even getting close to the randomized versions? In this paper, we give a negative answer to this question. We show that both Gaussian back substitution (GBS) and symmetric Gauss-Seidel (sGS) suffer from the same slow convergence issue as the cyclic order in the worst case. In particular, we prove that for unconstrained problems, both GBS-CD and sGS-CD can be $O(n^2)$ times slower than R-CD. Despite unconstrained problems, we also empirically study linearly constrained problems with quadratic objective: we empirically demonstrate that the convergence speed of GBS-ADMM and sGS-ADMM can be roughly $O(n^2)$ times slower than randomly permuted ADMM.

==> App1_update_matrix.tex <==


\section{Derivation of C-CD Iteration Matrix, for $n=3$}\label{appen: C-CD iteration matrix}
For completeness, we illustrate how to derive the expression 
of $\tilde{x}^k$ in GBS-CD used in the GBS-CD definition of Section \ref{subsec:alg_GBS} (this
derivation is same as the derivation of the update formula of C-CD for one iteration).
We consider a simple case with $n = 3, d_i = 1, \forall i$, and let $a_i = A_i \in \dR^{3 \times 1}$ and define $Q = A^TA$; the case for general $n$ is quite similar and omitted.

Recall the problem is to minimize a quadratic function:
\begin{equation}\label{least square optimization formulation, appen}
\begin{split}
  \min_{x \in \dR^n }  \quad   &    \frac{1}{2} \|Ax - b\|^2\\
\end{split}
\end{equation}

The update equations for the forward step can be written as
% the \textbf{prediction step} of GBS-CD at ($k+1$)-th iteration can be rewritten as
\begin{equation}\nonumber
\begin{split}
   & a_1^T(a_1 \tilde{x_1}^{k} + a_2 x_2^{k} + a_3 x_3^k - b) = 0, \\
   & a_2^T(a_1 \tilde{x_1}^{k} + a_2 \tilde{x_2}^{k} + a_3 x_3^k - b) = 0, \\
   & a_3^T(a_1 \tilde{x_1}^{k} + a_2 \tilde{x_1}^{k} + a_3 \tilde{x_3}^{k} - b ) = 0
\end{split}
\end{equation}
Denote $ \tilde{x}^{k}$ to be the updated iterate after the forward step in $k$-th iteration, then the above update equation becomes
\begin{equation}\label{iteration matrix of 123}
   \begin{bmatrix}
   a_1^T a_1 &     0     &      0     \\
   a_2^T a_1 & a_2^T a_2 &      0     \\
   a_3^T a_1 & a_3^T a_2 & a_3^T a_3  \\
   \end{bmatrix}
   \tilde{x}^{k} =
   \begin{bmatrix}
   0 & -a_1^T a_2 &  -a_1^Ta_3     \\
   0 &     0      &  -a_2^Ta_3     \\
   0 &     0      &      0         \\
   \end{bmatrix}
    x^k + 
    A^T b
\end{equation}

Define
\begin{equation}\label{eq:L123 3-block GBS}
 \Gamma \triangleq  \begin{bmatrix}
a_1^T a_1 &     0     &      0        \\
a_2^T a_1 & a_2^T a_2 &      0      \\
a_3^T a_1 & a_3^T a_2 & a_3^T a_3     \\
\end{bmatrix},  \quad
% R \triangleq  \begin{bmatrix}
% 0 & -a_1^T a_2 &  -a_1^Ta_3       \\
% 0 &     0      &  -a_2^Ta_3       \\
% 0 &     0      &      0           \\
% \end{bmatrix}.
\end{equation}
then we have  $  \Gamma \tilde{x}^{k}  = (  \Gamma - Q  ) x^k + A^T b  $.
This leads to 
$  \tilde{x}^{k}  = (I  - \Gamma^{-1} Q ) x^k + \Gamma^{-1}[A^T b].    $
 It is not hard to verify that the optimal solution $x^* = A^{-1}b $
 satisfies $ \Gamma^{-1}[A^T b] = x^* - (I  - \Gamma^{-1} Q )x^*  $,
 thus 
\begin{equation}
    \label{eq: appendix update of GBS-CD}
    \tilde{x}^{k} - x^*  = (I  - \Gamma^{-1} Q ) ( x^k - x^*).
\end{equation}
 
%  $  \tilde{x}^{k} - x^*  = (I  - \Gamma^{-1} Q ) ( x^k - x^*) .    $


==> sec1b_motivation.tex <==
\textbf{ADMM.} 
% CD methods are mainly used for unconstrained problems or constrained problems with uncoupled constraints. 
% in particular, to solve problem with linear constraints,
To solve large-scale problems with linear constraints, a natural idea is to combine CD methods with augmented Lagrangian method to obtain the so-called \rvs{ADMM algorithms}.
% so-called alternating direction method of multipliers (ADMM) 
\cite{glowinski1975approximation,chan1978finite,gabay1976dual,boyd2011distributed}.
Unlike CD where any reasonable update order can lead to convergence \cite{tseng2001convergence},
 for multi-block ADMM, even the most basic cyclic version does not converge \cite{chen2016direct}. 
% The counter-example given in \cite{chen2016direct}  is a simple problem of solving linear systems where 
% the objective function is 0 and the constraint is a 3-dimensional linear system of equations.
 Small \rvs{stepsize} versions of multi-block ADMM can be shown to converge with extra assumptions on the problem (see, e.g.
\cite{hong2012linear, han2012note,chen2013convergence,he2013proximal,he2013full, lin2014convergence,hong2014block,cai2014direct,sun2014convergent,lin2014global,han2014augmented,li2014schur,li2015convergent,lin2015iteration,deng2017parallel}), but the lesson from CD methods is that the speed advantage of CD exactly comes from large stepsize, thus we are more interested in ADMM with large \rvs{stepsize} (such
as \rvs{stepsize} $1$).

% More specifically, for the augmented Lagrangian function, ADMM iteratively performs coordinate descent for the primal variables and a gradient step for the dual variables.  
% ADMM was originally proposed in Glowinski and Marroco \cite{glowinski1975approximation} (see also Chan and Glowinski  \cite{chan1978finite}, Gabay and Mercier \cite{gabay1976dual}) for two blocks, 
% and  its extension to multiple blocks is straightforward \cite{chen2016direct}.

% ADMM has received significant attention recently because of its efficiency in solving large-scale
% constrained problems in statistics and machine learning \cite{boyd2011distributed}.

%to solve problem (1) when there are only two blocks (i.e. n = 2) and the objective function is separable
% ADMM catches researchers attentions because of its efficiency in solving problems in statistics and machine learning \cite{boyd2011distributed}.
% ADMM can be designed into parallel algorithms which are useful in solving large-scale problems in machine learning \cite{boyd2011distributed}. 

 
 
We are only aware of three major variants of multi-block ADMM with stepsize $1$ that are convergent
 in numerical experiments: Gaussian back substitution ADMM (GBS-ADMM) \cite{he2012alternating,he2012convergence},
symmetric Gauss-Seidel ADMM (sGS-ADMM) \cite{li2016schur,chen2017efficient} and randomly permuted ADMM (RP-ADMM) \cite{sun2015expected}. 
The first two use deterministic orders, and the third uses a random order. 
RP-ADMM is quite appealing since random permutation order is arguably the most popular update order for CD and SGD in practice.
% and appears as a standard choice in software frameworks (e.g. tensorflow). 
However, the theoretical analysis of random permutation is notoriously difficult even for CD and SGD \cite{recht2012beneath,sun2015expected,wright2017analyzing,lee2018random,gurbuzbalaban2015random,gurbuzbalaban2018randomness},
and for RP-ADMM only the expected convergence for quadratic objective function is known \cite{sun2015expected, chen2015convergence}.
% convergence for general convex problems remains open.
In contrast, GBS-ADMM enjoys strong theoretical guarantee as the convergence for separable 
convex objective with linear constraints is proved \cite{he2012alternating}.
For sGS-ADMM, the convergence guarantee is proved for a sub-class of convex problems. 
% separable
% In short, there are stronger theoretical convergence guarantee for
% sGS-ADMM and GBS-ADMM than RP-ADMM. 

If our purpose is just to resolve the divergence issue of cyclic ADMM,
then GBS-ADMM and sGS-ADMM both provide rather satisfactory (though not perfect) theoretical guarantee on the convergence.
However, the major purpose of using block decomposition is to solve large-scale problems, thus
the convergence speed is also very important.
% When it comes to convergence speed, 
What can we say about the convergence speed of GBS-ADMM and sGS-ADMM? 
Are they provably faster the one-block version, just like R-CD \cite{nesterov2012efficiency, leventhal2010randomized}? 
To understand GBS-ADMM and sGS-ADMM, we need to first understand the case when GBS and sGS update orders are applied to unconstrained problems.
% To understand GBS-ADMM and sGS-ADMM, we need to first understand their unconstrained counter-parts GBS-CD and sGS-CD.


% Does the strong convexity of the objective function guarantee fast convergence speed of GBS-ADMM and sGS-ADMM?

%------
% Before answering the questions, one needs to first answer a simpler question:
% are GBS-ADMM and sGS-ADMM always fast on unconstrained problems? 
% As this question is still open,  we will focus on the unconstrained counter-parts of the two algorithms. % , which are variants of CD methods. 
%------

% Similar to CD, a desirable result would be that GBS-ADMM and sGS-ADMM are 1 to $n$ times
% faster than the single-block algorithm  ALM (augmented Lagrangian method).
% However, this result would imply that for unconstrained problems 
% (a special case of constrained problems with no constraint),
% there exists a deterministic variant of CD that is 1 to $n $ times faster than GD.
% Thus there are two extreme possibilities:
% one possibility is that we answer the open question on the existence of fast
% deterministic CD, and another possibility is that
% GBS-ADMM and sGS-ADMM can be very slow in the worst case.
% Either possibility will improve our understanding of the problems. Which possibility is closer to the truth? 

%  on the fast deterministic variant of CD, GBS-ADMM and sGS-ADMM are always much faster than ALM in theory



% a ``batch'' method 
% In light of the recent results on C-CD and R-CD, 

% Both GBS-ADMM and sGS-ADMM are based on the idea of symmetrization. 

% The convergence of sGS-ADMM is only proved for a sub-class of convex problems, but still a bigger class than the quadra 
% As for RP-ADMM, only a weaker notion of convergence is established for R
% As for RP-ADMM, convergence result is established for RP-ADMM \cite{sun2015expected,chen2015convergence},

%  \cite{recht2012beneath}. 











